Cue-CoT: Chain-of-thought Prompting for Responding to In-depth Dialogue Questions with LLMs

Large Language Models (LLMs), such as \texttt{ChatGPT}, greatly empower dialogue systems with strong language understanding and generation capabilities. However, most of the previous works prompt the LLMs to directly generate a response based on the dialogue context, overlooking the underlying linguistic cues about the user status exhibited in the context. Such in-depth dialogue scenarios are challenging for existing LLMs to figure out the user's hidden needs and respond satisfactorily through a single-step inference. To this end, we propose a novel linguistic cue-based chain-of-thoughts (\textit{Cue}-CoT), which enhances the LLMs inference with an intermediate reasoning step to find cues exhibited in the dialogue, aiming to provide a more personalized and engaging response. To evaluate the approach, we build a benchmark with in-depth dialogue questions, consisting of 6 datasets in both Chinese and English, targeting 3 major linguistic cues during the conversation: \textit{personality}, \textit{emotion}, and \textit{psychology}. We conduct extensive experiments on the proposed benchmark with 5 LLMs under both zero-shot and one-shot settings. Empirical results demonstrate our proposed \textit{Cue}-CoT method outperforms standard prompting methods in terms of both \textit{helpfulness} and \textit{acceptability} on all datasets.

==> tables/main_cn.tex <==
\begin{table*}[!t]
    \centering
    \begin{adjustbox}{max width=1.0\textwidth}
    \begin{tabular}{l|cccc|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{CoT}} & \multicolumn{4}{|c}{\textbf{Explicit CoT}} \\
    \cline{2-9} & \textbf{Zhihu} & \textbf{D4} & \textbf{PsyQA} & \textbf{Sum} & \textbf{Zhihu} & \textbf{D4} & \textbf{PsyQA} & \textbf{Sum} \\
    \hline
    \hline
    \multicolumn{9}{c}{\textit{\textbf{Zero-shot Setting}}} \\
    \hline
    \hline
    \textsc{belle-llama-7b-2m} & 67.40 & 76.34 & 69.31 & 70.98 & 81.54 (60.23) & 71.60 (72.41)  & 79.25 (73.65) & 77.76 \\
    \textsc{chatglm-6b} & 48.29 & 56.68 & 33.00 & 45.99 & 85.02 (66.67) & 72.10 (51.27) & 83.57 (55.40) & 80.24 \\
    \textsc{chatgpt} & 67.91 & 50.40 & 61.90 & 60.10 & 95.57 (65.22) & 87.88 (61.08) & 90.34 (56.12) & 91.27 \\
    \hline
    \hline
    \multicolumn{9}{c}{\textit{\textbf{One-shot Setting}}}  \\
    \hline
    \hline
    \textit{\textbf{random}} \\
    \hdashline 
    \textsc{belle-llama-7b-2m}  & 64.31 & \underline{50.53} & 65.15 & 61.53 & 83.30 & \underline{69.59} & 73.81 & 77.32  \\
    \textsc{chatglm-6b}  & - & - & - & - & 90.28 & 75.10 & 91.85 & 85.70 \\
    \textsc{chatgpt}  & 76.47 & 51.94 & 65.44 & 64.65 & 91.60 & 86.67 & 88.96 & 89.10 \\
    \hline
    \textit{\textbf{top-1}}  \\
    \hdashline 
    \textsc{belle-llama-7b-2m} & 63.77 & \underline{57.51} & 69.92 & 64.81 & 82.77 & \underline{69.94} & 73.99 & 77.24 \\
    \textsc{chatglm-6b} & - & - & - & - & 89.25 & 77.26 & 91.77 & 86.09 \\
    \textsc{chatgpt} & 76.86 & 50.93 & 55.85 & 61.33 & 93.19 & 88.84 & 91.77 & 91.30 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The win rate of responses generated by \textbf{CoT} and \textbf{Explicit CoT} compared with the response with standard prompting on three \textbf{Chinese} datasets in terms of \textbf{helpfulness}. The \underline{underlined} numbers mean that there are about 160 valid responses out of 500 in this setting due to the input context limit of the model.}
    \label{tab:main_cn}
\end{table*}

==> tables/main_en.tex <==
\begin{table*}[!t]
    \centering
    \begin{adjustbox}{max width=1.0\textwidth}
    \begin{tabular}{l|cccc|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{CoT}} & \multicolumn{4}{|c}{\textbf{Explicit CoT}} \\
    \cline{2-9} & \textbf{Quora} & \textbf{ED} & \textbf{EMH} & \textbf{Sum} & \textbf{Quora} & \textbf{ED} & \textbf{EMH} & \textbf{Sum} \\
    \hline
    \hline
    \multicolumn{9}{c}{\textit{\textbf{Zero-shot Setting}}} \\
    \hline
    \hline
    \textsc{flan-t5-xxl} & 60.45 & 53.85 & \underline{55.49} & 56.72 & 63.58 (52.14) & 55.17 (55.24) & \underline{58.61} (55.56) & 59.20 \\
    \textsc{alpaca-7b} & 19.51 & 35.41 & \underline{49.70} & 33.11 & 80.78 (78.21) & 87.30 (86.00) & \underline{85.76} (86.97) & 84.49\\
    \textsc{vicuna-7b-v1.1} & 56.16 & 71.43 & \underline{59.23} & 62.65 & 81.67 (77.89) & 91.30 (90.71) & \underline{80.42} (82.93) & 84.97\\
    \textsc{chatgpt} & 79.47 & 88.31 & \underline{82.93} & 83.66 & 85.83 (89.09) & 91.98 (96.79) & 82.83 (94.93) & 87.08 \\
    \hline
    \hline
    \multicolumn{9}{c}{\textit{\textbf{One-shot Setting}}}  \\
    \hline
    \hline
    \textit{\textbf{random}} \\
    \hdashline 
    \textsc{flan-t5-xxl} & - & - & - & - & 59.32 & 56.00 & \underline{61.42} & 58.61 \\
    \textsc{alpaca-7b} & - & - & - & - & 76.78 & 85.08 & \underline{94.36} & 84.37\\
    \textsc{vicuna-7b-v1.1} & 60.45 & 70.77 & \underline{63.06} & 64.98 & 79.84 & 91.20 & \underline{79.23} & 83.95 \\
    \textsc{chatgpt} &80.33 & 87.32 & \underline{84.94} & 84.13 & 84.31 & 89.78 & \underline{85.71} & 86.71 \\
    \hline
    \textit{\textbf{top-1}}  \\
    \hdashline 
    \textsc{flan-t5-xxl} & - & - & - & - & 64.93 & 62.00 & \underline{59.05} & 62.35 \\
    \textsc{alpaca-7b} & - & - & - & - & 74.54 & 78.70 & \underline{88.69} & 79.79 \\
    \textsc{vicuna-7b-v1.1} & 63.10 & 71.75 & \underline{62.31} & 66.11 & 78.70 & 90.12 & \underline{79.10} & 83.08 \\
    \textsc{chatgpt} & 81.15 & 87.42 & \underline{81.40} & 83.58 & 88.08 & 91.37 & \underline{86.87} & 89.01 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The win rate of responses generated by \textbf{CoT} and \textbf{Explicit CoT} compared with the response with standard prompting on three \textbf{English} datasets in terms of \textbf{helpfulness}. The \underline{underlined} numbers mean that there are about 330 valid responses out of 500 in this setting due to the input context limit of the model.}
    \label{tab:main_en}
\end{table*}

==> tables/w_groud_truth_cn.tex <==
\begin{table*}[!t]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l|cc|cc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Zhihu}} & \multicolumn{2}{c|}{\textbf{PsyQA}} & \multicolumn{2}{c}{\textbf{D4}}  \\
     \cline{2-7}  & Help. & Acce. & Help. & Acce. & Help. & Acce. \\
    \hline
    \textsc{chatglm-6b} & 86.63 & 86.67 & 70.12 & 74.35 & 90.91 & 92.81 \\
    \textsc{pangu-$\alpha$-6b} \\
    \textsc{belle-llama-7b-2m} & 74.16 & 75.71 & 44.17  &  45.75 & 89.18 & 87.23 \\
    \textsc{gpt-3.5-turbo} & 81.36 & 88.46 & 83.19 & 84.93 & 94.10 & 94.15 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The win rate of responses generated by our method compared with the ground truth on three \textbf{Chinese} datasets.}
    \label{tab:main_exp}
\end{table*}

==> tables/w_ground_truth_en.tex <==
\begin{table*}[!t]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l|cc|cc|cc}
    \toprule
    \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Quora}} & \multicolumn{2}{c|}{\textbf{ED}} & \multicolumn{2}{c}{\textbf{EMH}}  \\
     \cline{2-7}  & Help. & Acce. & Help. & Acce. & Help. & Acce. \\
    \hline
    \textsc{flan-t5-xxl} & \\
    \textsc{alpaca-7b} & 69.57 & 65.93 & 96.81 & 97.85 & 72.83 & 76.09 \\
    \textsc{vicuna-7b-v1.1} & 96.77 & 92.47 & 100 & 100 & 98.90 & 97.80 \\
    \textsc{gpt-3.5-turbo} & 96.94 & 97.00 & 98.99 & 99.00 & 97.94 & 98.97 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The win rate of responses generated by our method compared with the ground truth on three \textbf{English} datasets.}
    \label{tab:main_exp}
\end{table*}
